Self Contrastive Learning for Session-based Recommendation

Session-based recommendation, which aims to predict the next item of users' interest as per an existing sequence interaction of items, has attracted growing applications of Contrastive Learning (CL) with improved user and item representations. However, these contrastive objectives: (1) serve a similar role as the cross-entropy loss while ignoring the item representation space optimisation; and (2) commonly require complicated modelling, including complex positive/negative sample constructions and extra data augmentation. In this work, we introduce Self-Contrastive Learning (SCL), which simplifies the application of CL and enhances the performance of state-of-the-art CL-based recommendation techniques. Specifically, SCL is formulated as an objective function that directly promotes a uniform distribution among item representations and efficiently replaces all the existing contrastive objective components of state-of-the-art models. Unlike previous works, SCL eliminates the need for any positive/negative sample construction or data augmentation, leading to enhanced interpretability of the item representation space and facilitating its extensibility to existing recommender systems. Through experiments on three benchmark datasets, we demonstrate that SCL consistently improves the performance of state-of-the-art models with statistical significance. Notably, our experiments show that SCL improves the performance of two best-performing models by 8.2% and 9.5% in P@10 (Precision) and 9.9% and 11.2% in MRR@10 (Mean Reciprocal Rank) on average across different benchmarks. Additionally, our analysis elucidates the improvement in terms of alignment and uniformity of representations, as well as the effectiveness of SCL with a low computational cost.

==> paper/tmp_experiment_2.tex <==
\section{Sequential Recommendation with User Profiles}
\label{sec:rec_with_user_profile}

\subsection{Setup}
\paragraph{\textbf{Datasets.}} 
\input{table/dataset_statistics_2}
The experiments are conducted over five benchmark datasets with statistics after preprocessing shown in Table~\ref{tab:datasets}.
\begin{itemize}
    \item \textbf{Amazon Beauty}, \textbf{Clothing} and \textbf{Sports}~\cite{amazon}\footnote{http://jmcauley.ucsd.edu/data/amazon/}. Following baselines~\cite{kang2018self,bert4rec,s3-rec,xie2022contrastive,duorec2022}, the widely used Amazon dataset is chosen in our experiments with three sub-categories.
    \item \textbf{MovieLens-1M}~\cite{movielens}\footnote{https://grouplens.org/datasets/movielens/1m/}. Following~\cite{bert4rec}, the popular movie recommendation dataset is used here, denoted as ML-1M.
    \item \textbf{Yelp}\footnote{https://www.yelp.com/dataset}, which is a widely used dataset for the business recommendation. Similar to~\cite{s3rec}, the transaction records after Jan. 1st, 2019 are used in our experiment.
\end{itemize}

\paragraph{\textbf{Baselines.}} 
\label{sec:baseline_2}
The following methods are used for comparison:
\begin{itemize}
    \item \textbf{BPR-MF} \cite{bprmf} is the first method to use the Bayesian Personalized Ranking (BPR) loss function to train a matrix factorization model for sequential recommendation.
    \item \textbf{GRU4Rec} \cite{hidasi2015session} is the first recurrent model for sequential recommendation, which applies Gated Recurrent Unit (GRU) to model the user sequence.
    \item \textbf{Caser}~\cite{tang2018caser} is a Convolutional Neural Network (CNN) based method that captures high-order patterns by applying horizontal and vertical convolutional operations for sequential recommendation.
    \item \textbf{SASRec}~\cite{kang2018self} is a single-directional self-attention model, which is a strong baseline for sequential recommendation.
    \item \textbf{BERT4Rec}~\cite{bert4rec}  is a sequential recommendation model that uses BERT \cite{devlin2018bert} as the backbone and employs a masked item training scheme similar to the masked language modelling.
    \item \textbf{$\text{S}^3\text{Rec}$}~\cite{s3-rec} is a sequential recommendation model that uses masked contrastive pre-training and the variant of Mask Item Prediction (MIP).
    \item \textbf{CL4SRec}~\cite{xie2022contrastive} is a sequential recommendation model that uses item cropping, masking, and reordering as augmentations for contrastive learning.
    \item \textbf{DuoRec}~\cite{duorec2022} a sequential recommendation model that aims to improve the quality of item embeddings and sequence representations. However, it relies on additional methods such as data augmentation and positive/negative sampling to achieve its goals.
\end{itemize}



\paragraph{\textbf{Evaluation Metrics.}}
The authors follow the protocols established in previous works~\cite{kang2018self,bert4rec,s3-rec,xie2022contrastive,duorec2022}, where the last interacted item of each user sequence is used for testing, the second last item is used for validation, and all earlier items are used for training. The predicted next item is chosen from the pool of all items without any candidate filter. 
Our experiments compare the different methods using two metrics, Hit Ratio at $k$ (HR@$k$) and Normalized Discounted Cumulative Gain at $k$ (NDCG@$k$) with $k$ chosen from {5,10}.

\paragraph{\textbf{Implementation Details.}}
%
Following previous studies such as ~\cite{kang2018self,bert4rec,s3-rec,xie2022contrastive,duorec2022}, the authors adopt the same preprocessing techniques and consider all interactions as implicit feedback. Users or items that appear less than five times are removed, and the maximum length of a sequence is set at 50.
% DuoRec \cite{duorec2022} was proposed to improve the item embeddings and sequence representations. However, it relies on extra augmentation method and positive/negative sampling method. 

% CL4SRec \cite{xie2022contrastive}
% \cite{10.1145/3511808.3557317} leveraged contrastive learning by learning items’ importance in a user sequence to derive the positive and negative sequences accordingly.

\subsection{Experimental Results}
\input{table/baseline2}
We propose a more efficient method without depending on these sophisticated methods. However, its results cannot be reproduced and received many complaints on its github repository. 


The table above shows the overall performance of different methods on three datasets (Beauty, Clothing, and Sports). The metric used in this table is HR@K and NDCG@K with K = 5 and 10. The bold scores represent the highest results of all methods. The methods such as BPR-MF, GRU4Rec, Caser, SASRec, BERT4Rec, and $\text{S}^3\text{Rec}$ are the traditional methods, while CL4SRec, w/ SCL, DuoRec and w/ SCL are the proposed methods in this research.

In the Beauty dataset, the proposed method w/ SCL achieves the highest HR@5, HR@10, NDCG@5, and NDCG@10 scores among all methods. In the Clothing dataset, the proposed method w/ SCL also achieves the highest HR@5, HR@10, NDCG@5, and NDCG@10 scores among all methods. In the Sports dataset, the proposed method w/ SCL also achieves the highest HR@5, HR@10, NDCG@5, and NDCG@10 scores among all methods.

In overall, the proposed method w/ SCL has achieved the best results in all the three datasets, showing the effectiveness of the Self-Contrastive Learning method in the recommendation task.

Based on the results in the table, the method "CL4SRec w/ SCL" outperforms all other methods in terms of Hit Ratio (HR@5, HR@10) and Normalized Discounted Cumulative Gain (NDCG@5, NDCG@10) on the Beauty, Clothing and Sports datasets.

On the Beauty dataset, it has the highest HR@5 and HR@10 scores of 0.0552 and 0.0846 respectively. The NDCG@5 and NDCG@10 scores are also the highest with 0.0345 and 0.0439 respectively. The improvement in scores compared to the other methods is relatively significant.

On the Clothing dataset, it has the highest HR@5 and HR@10 scores of 0.0193 and 0.0300 respectively. The NDCG@5 and NDCG@10 scores are also the highest with 0.0105 and 0.0140 respectively. The improvement in scores compared to the other methods is relatively significant.

On the Sports dataset, it has the highest HR@5 and HR@10 scores of 0.0309 and 0.0475 respectively. The NDCG@5 and NDCG@10 scores are also the highest with 0.0248 and 0.0370 respectively. The improvement in scores compared to the other methods is relatively significant.

In summary, the results show that SCL method is able to significantly improve the performance of the CL4SRec method on all datasets, achieving the best results among all methods.


The table provides the overall performance of various methods on three datasets, Beauty, Clothing, and Sports. It can be seen that the proposed SCL method, when applied to the CL4SRec and DuoRec models, improves the performance in terms of Hit Ratio (HR@5, HR@10) and Normalized Discounted Cumulative Gain (NDCG@5, NDCG@10) on all three datasets. Specifically, on the Beauty dataset, SCL improves the HR@5 and HR@10 by 1.4\% and 3.6\%, respectively, and NDCG@5 and NDCG@10 by 1.8\% and 3.4\%. On the Clothing dataset, SCL improves the HR@5 and HR@10 by 2.8\% and 6.7\%, respectively, and NDCG@5 and NDCG@10 by 4.2\% and 4.2\%. On the Sports dataset, SCL improves the HR@5 and HR@10 by 2.7\% and 4.1\%, respectively, and NDCG@5 and NDCG@10 by 2.9\% and 3.7\%. Overall, the results demonstrate that SCL is effective in improving the performance of existing recommendation approaches on those three datasets.

We only evaluated our SCL method on the DuoRec model because it had a significant performance advantage over CL4SRec.

==> table/dataset_statistics.tex <==
\begin{table}[t!]
\centering
\scriptsize
\caption{Statistics of datasets.}
% \vspace{-0.8em}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{lccc}
\toprule
\bf  Dataset         & \bf \tmall    & \bf \nowplaying & \bf \diginetica \\ \midrule
Train Size      & 351,268  & 825,304    & 719,470 \\
Test Size       & 25,898   & 89,824     & 60,858 \\
Items Size      & 40,728   & 60,417     & 43,097 \\
Average Length  & 6.69     & 7.42       & 5.12 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{table:dataset1}
\end{table}
